On the Benefit of Generative Foundation Models for Human Activity Recognition

In human activity recognition (HAR), the limited availability of annotated data presents a significant challenge. Drawing inspiration from the latest advancements in generative AI, including Large Language Models (LLMs) and motion synthesis models, we believe that generative AI can address this data scarcity by autonomously generating virtual IMU data from text descriptions. Beyond this, we spotlight several promising research pathways that could benefit from generative AI for the community, including the generating benchmark datasets, the development of foundational models specific to HAR, the exploration of hierarchical structures within HAR, breaking down complex activities, and applications in health sensing and activity summarization.

==> figure/f1_per_cls.tex <==
% \begin{figure}
%     \centering
%     \vspace{-0.09in}
%     \subfigure[]{\includegraphics[width=.6\linewidth]{figure/f1_per_cls_fig.pdf}
%     \label{fig:f1_per_cls}
%     }
%     % \hfill
%     \subfigure[]{\includegraphics[width=.33\linewidth]{figure/waiting.png}
%     \label{fig:lying_vis}
%     }
%     \vspace*{-1.7em}
%         \caption{(a) Differences in F1 score for each activity between the classifier trained on only real IMU data and the classifier trained on both real and virtual IMU data evaluated on the RealWorld \cite{Sztyler2016realworld} dataset. (b) Example where the motion synthesis model confused waiting with lying. }
%     \label{fig:discussion}

%   %  \vspace*{-1.5em}
    
% \end{figure}

\begin{figure}
    \centering
    \vspace{-0.15in}
    \subfloat[]{\includegraphics[width=.53\linewidth]{figure/f1_per_cls_fig.pdf}
    \label{fig:f1_per_cls}
    }
    % \hfill
    \subfloat[]{\includegraphics[width=.29\linewidth]{figure/waiting.png}
    \label{fig:lying_vis}
    }
    \vspace*{-1.3em}
        \caption[]{(a) Differences in F1 score for each activity between the classifier trained on only real IMU data and the classifier trained on both real and virtual IMU data evaluated on the RealWorld \cite{Sztyler2016realworld} dataset. (b) Example where the motion synthesis model confused waiting with lying. }
    \label{fig:discussion}

   \vspace*{-0.4em}
    
\end{figure}

==> figure/f1_vary_real.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=.80\linewidth]{figure/f1_vary_real_figure.pdf}
    \vspace{-0.1in}
    \caption{ Model performance on RealWorld \cite{Sztyler2016realworld}, PAMAP2 \cite{Reisspamap}, and USC-HAD \cite{Zhang2012usc} datasets when different amount of real IMU data are used for training. The amount of virtual IMU data used remains the same. 
    }
    \label{fig:vary_imu}

    \vspace{-0.2in}
\end{figure*}

==> figure/imutube.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=.9\linewidth]{figure/extended_imutube.pdf}
    \vspace{-0.1in}
    \caption{
    IMUTube queries video data from repositories like YouTube using activity keywords. The Adaptive Video Selection module filters out segments prone to poor 3D motion tracking due to noise, occlusions, or motion blur. The remaining videos are used to estimate 3D human motion, virtual IMU data is then extracted and calibrated with real sensor data.
    (Figure adopted from Kwon \etal \cite{kwon2021complex} and used with permission). 
    }
    \vspace{-0.2in}
    \label{fig:imutube}
\end{figure*}

==> sections/limitation/main.tex <==
\vspace{-0.1in}
\section{Limitations of Existing Approaches}
\noindent
While both video and text-based systems have proven effective in generating virtual IMU data to enhance downstream HAR model performance, they are not without limitations. In this section, we explore the constraints of both approaches, with a particular focus on IMUTube for video based systems, and suggest potential future directions to increase their utility.


\vspace{-0.1in}
\subsection{IMUTube}

IMUTube was initially designed for and tested on activities involving locomotion and gym exercises, which typically involve large body movements and coarser motion patterns. However, a recent study \cite{leng2022finegrained} assessed IMUTube's performance on daily activities characterized by subtler motion patterns. The results showed that the virtual IMU data generated for these daily activities were essentially noise and led to degraded performance of the downstream classifiers.

This issue primarily arises due to the limitations of the computer vision methods employed in IMUTube, which struggle to capture the nuances of subtle motion. Naturally, a straightforward way to enhance IMUTube is by upgrading the computer vision methods within it. Since the inception of IMUTube, the state-of-the-art in computer vision, particularly in 2D/3D pose estimation -argubaly the most critical aspect of IMUTube— has evolved considerably. The current state-of-the-art methods in this domain are ViTPose \cite{xu2022vitpose} and MotionBERT \cite{motionbert2022}, both of which outperform the pose estimation methods previously used in IMUTube, namely AlphaPose \cite{alphapose} and VideoPose3D \cite{pavllo:videopose3d:2019}. Improved pose estimation methods would result in less noisy poses and consequently higher-quality virtual IMU data. 

Additionally, IMUTube struggles with videos that have significant camera ego-motion. This issue arises because most existing 3D pose estimation methods, including MotionBERT and VideoPose3D, output the 3D human pose in the camera frame rather than the world frame. In videos with significant camera ego-motion, such as a camera following a soccer player, the estimated 3D human motion often suffers from poor global motion estimation. This is because the 3D human pose estimation model does not account for the human's position in the world frame. Such inaccuracies in global motion estimation can reduce the quality of the generated virtual IMU data. Fortunately, the recent introduction of SLAHMR \cite{ye2023slahmr}, the first 3D pose estimation method to output poses in the world frame, offers a solution. By using SLAHMR, global human motion can be retained even in videos with significant camera ego-motion, expanding the applicability of IMUTube to a wider range of videos.

Lastly, IMUTube makes the assumption that every human in the input video is engaged in the desired activity. This is not always a reasonable assumption, as videos can include other individuals engaged in unrelated activities, or even worse, no one in the video may be performing the intended activity. In such cases, the virtual IMU data generated for the unwanted activities could adversely affect the performance of the downstream classifier. We propose two potential solutions to address this issue: referring video object segmentation (RVOS) \cite{li2022r} and vision-based action recognition \cite{motionbert2022}. RVOS involves segmenting objects in a video based on a textual description. For instance, given the prompt "a person is walking," an RVOS model would generate masks indicating where the walking person is in the video, or produce no masks if no one is walking in the video. Alternatively, vision-based action recognition methods use human poses, either in 2D or 3D, as input to determine the activity being performed. These approaches would enable IMUTube to identify which individuals, if any, are performing the desired activity in the video.

\input{tables/prompts}

\vspace{-0.13in}
\subsection{Text Based System}
The motion synthesis model, T2M-GPT, employed by the text-based system, is trained on the HumanML3D dataset—a substantial collection of 3D human motion data accompanied by textual descriptions. However, T2M-GPT has limitations in generating human motion sequences for activities that are not represented in the HumanML3D dataset. Moreover, the generated human motion sequences lack facial and hand motions. A cost-effective solution to overcome these limitations would be to augment the training dataset with new activities. This can be achieved by utilizing computer vision techniques such as 3D human pose estimation \cite{ye2023slahmr} to extract human motion sequences for new activities from existing videos. The recently introduced Motion-X dataset \cite{lin2023motionx} demonstrates this approach. Motion-X collects motion sequences from various public datasets and extracts additional human motion sequences from online videos. It contains 95,642 clips of motion sequences along with their corresponding textual descriptions, making it six times larger than the HumanML3D dataset and covering a broader range of activities. Furthermore, the Motion-X dataset incorporates facial and hand motions. The ability to generate hand motion could be particularly beneficial for fine-grained activities such as typing and writing, which involve minimal wrist motion. Facial motion and facial virtual IMU data might also be useful for earables and smart glasses.

Lastly, T2M-GPT occasionally struggles with distinguishing closely related activities or correctly interpreting prompts with multiple verbs. For instance, the model may confuse "climbing up stairs" with "climbing down stairs," or misinterpret "walking forward," "walking clockwise," and "walking counterclockwise." Additionally, when confronted with a prompt containing two or more verbs, the model may incorrectly prioritize one verb over the other. Take the example prompt "a person rests flat on their backs, arms stretched out above their head." In this case, the model might focus on "stretched out" instead of "rests flat," producing a human motion sequence resembling standing and stretching rather than lying down. To mitigate these issues, we suggest exploring alternative motion synthesis models, such as MotionDiffuse \cite{zhang2022motiondiffuse}, SINC \cite{SINC:ICCV:2022}, and MotionGPT \cite{jiang2023motiongpt}, to assess if they exhibit fewer such problems.

==> tables/dataset.tex <==
\begin{table}
\centering
    \caption{Real and virtual IMU datasets size for the three HAR datasets we used for evaluation. 
    }
    \vspace*{-1.0em}
    \begin{adjustbox}{width=0.55\columnwidth,center}
    \begin{tabular}{c|c|c}
        Dataset & Real Size & Virtual Size \\
         \hline\hline
        RealWorld & 1,107 min & 41 min\\ 
         \hline
         PAMAP2  &  322 min & 68 min \\
         \hline
          USC-HAD &  469 min & 69 min \\
%         \hline
    \end{tabular}
    \end{adjustbox}
    \label{tab:dataset}
    %\vspace*{-0.5em}
    % \vspace{-0.2in}
\end{table}

==> tables/f1_mode.tex <==

\begin{table}
\centering
\caption{Model performances (Macro F1) for the experimental evaluation of our approach for  the three HAR datasets. 
% The best performance within each scenario is highlighted in bold.
}
\vspace{-0.25cm}

\subfloat[Random Forest]{
\begin{adjustbox}{width=0.85\columnwidth,center}
    \begin{tabular}{c|c|c|c}
         Dataset & PAMAP2 & RealWorld & USC-HAD\\
         \hline\hline
         Real & $0.659 \pm 0.003$ & $0.715 \pm 0.011$ & $0.478 \pm 0.002$\\
         \hline
         Virtual & $0.628 \pm 0.003$ & $0.746 \pm 0.003$   & $0.448 \pm 0.003$ \\
         \hline
         Real+Virtual & $\textbf{0.699} \pm 0.004$ & $\textbf{0.770} \pm 0.004$ & $\textbf{0.486} \pm 0.003$ \\
        \hline
    \end{tabular}
    \end{adjustbox}

}

\vspace{-0.25cm} 
\subfloat[DeepConvLSTM]{
\begin{adjustbox}{width=0.85\columnwidth,center}
    \begin{tabular}{c|c|c|c}
         Dataset & PAMAP2 & RealWorld & USC-HAD\\
         \hline\hline
         Real & $0.687 \pm 0.008$ & $0.796 \pm 0.015$ & $\textbf{0.646} \pm 0.008$\\
         \hline
         Virtual & $0.626 \pm 0.015$ & $0.681 \pm 0.005$   & $0.453 \pm 0.008$ \\
         \hline
         Real+Virtual & $\textbf{0.723} \pm 0.007$ & $\textbf{0.820} \pm 0.002$ & $0.640 \pm 0.002$ \\
        \hline
    \end{tabular}
    \end{adjustbox}

}
\vspace*{-1em}
 \label{tab:results}
\end{table}




==> tables/f1_sensor.tex <==
 \begin{table}[t]
    \centering
    \vspace{-0.in}
    \caption{Model performances on the RealWorld dataset \cite{Sztyler2016realworld} for various scenerios. SMPL indicates the joints' rotations extracted by fitting joint positions to a SMPL model during virtual IMU data generation. IK indicates inverse kinematics is used during generation. The best performance within each scenario bolded. \thomas{2 digits after the decimal point are enough.} \zikang{I changed it to 3 digits to make sure that the confidence interval is not 0. }
    }
    \begin{adjustbox}{width=\columnwidth,center}
    \begin{tabular}{c|c|c|c|c}
          Sensors & Real Size & Dataset & F1  (SMPL) & F1 (IK) \\
         \hline\hline
         \multirow{6}{*}{Forearm} 
         & \multirow{3}{*}{110 minutes} & Real & $0.444 \pm 0.004$ &  $0.444 \pm 0.004$\\
         \cline{3-5}
         & & Virtual & $0.573 \pm 0.003$ & $0.523 \pm 0.003$ \\
         \cline{3-5}
         & & Real + Virtual & $0.589 \pm 0.005$ & $\textbf{0.602} \pm 0.012$\\
         \cline{3-5}
         \hhline{~====}
         & \multirow{3}{*}{1107 minutes} & Real & $0.613 \pm 0.006$ & $0.613 \pm 0.006$\\
         \cline{3-5}
         & & Virtual & $0.573 \pm 0.003$ & $0.523 \pm 0.003$  \\
         \cline{3-5}
         & & Real +Virtual & $\textbf{0.624} \pm 0.006$ & $0.620 \pm 0.002$ \\
         \cline{3-5}
         \hline\hline
         \multirow{6}{*}{All 7 sensors} 
          & \multirow{3}{*}{110 minutes} & Real & $0.481 \pm 0.009$ & $0.481 \pm 0.009$ \\
         \cline{3-5}
         & & Virtual & $0.752 \pm 0.003$ & $0.746 \pm 0.003$  \\
         \cline{3-5}
         & & Real + Virtual & $\textbf{0.776} \pm 0.008$ & $0.758 \pm 0.011$ \\
         \cline{3-5}
         \hhline{~====}
         & \multirow{3}{*}{1107 minutes} & Real & $0.715 \pm 0.011$ & $0.715 \pm 0.011$\\
         \cline{3-5}
         & & Virtual & $0.757 \pm 0.011$ & $0.746 \pm 0.003$  \\
         \cline{3-5}
         & & Real +Virtual & $0.769 \pm 0.004$ & $\textbf{0.770} \pm 0.004$ \\
         \cline{3-5}
         \hline
    \end{tabular}
    \end{adjustbox}
    \label{tab:results}
    \vspace{-0.08in}
\end{table}

==> tables/f1_usc_had.tex <==
 \begin{table}[t]
    \centering
    \vspace{-0.in}
    \caption{Model performances on the USC-HAD \cite{Zhang2012usc} dataset. The best performance within each scenario bolded.
    }
    \begin{adjustbox}{width=0.6\columnwidth,center}
    \begin{tabular}{c|c|c}
          Real Size & Dataset & F1 Score \\
         \hline\hline
          \multirow{3}{*}{47 minutes} & Real 
         & $0.399 \pm 0.004$ \\
         \cline{2-3}
         & Virtual & $0.448 \pm 0.003$  \\
         \cline{2-3}
         & Real + Virtual & $\textbf{0.471} \pm 0.009$ \\
         \hline\hline
         \multirow{3}{*}{469 minutes} & Real 
         & $0.478 \pm 0.002$ \\
         \cline{2-3}
        &  Virtual & $0.448 \pm 0.003$  \\
         \cline{2-3}
         & Real +Virtual & $\textbf{0.486} \pm 0.003$  \\
         \cline{2-3}
         \hline
    \end{tabular}
    \end{adjustbox}
    \label{tab:usc-had}
    \vspace{-0.08in}
\end{table}
